Scientific Open-Source Software Is Less Likely to Become Abandoned Than One Might Think! Lessons from Curating a Catalog of Maintained Scientific Software

Scientific software is essential to scientific innovation and in many ways it is distinct from other types of software. Abandoned (or unmaintained), buggy, and hard to use software, a perception often associated with scientific software can hinder scientific progress, yet, in contrast to other types of software, its longevity is poorly understood. Existing data curation efforts are fragmented by science domain and/or are small in scale and lack key attributes. We use large language models to classify public software repositories in World of Code into distinct scientific domains and layers of the software stack, curating a large and diverse collection of over 18,000 scientific software projects. Using this data, we estimate survival models to understand how the domain, infrastructural layer, and other attributes of scientific software affect its longevity. We further obtain a matched sample of non-scientific software repositories and investigate the differences. We find that infrastructural layers, downstream dependencies, mentions of publications, and participants from government are associated with a longer lifespan, while newer projects with participants from academia had shorter lifespan. Against common expectations, scientific projects have a longer lifetime than matched non-scientific open-source software projects. We expect our curated attribute-rich collection to support future research on scientific software and provide insights that may help extend longevity of both scientific and other projects.

==> Inspirations/Goodlinks.tex <==
https://www.sciencedirect.com/science/article/pii/S0164121218301468
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8816759&tag=1
https://dl.acm.org/doi/pdf/10.1145/3379597.3387495
https://drive.google.com/file/d/1MUgVNFi9QZ2iobqzJq7mS3Ef8ZfmDkCy/view?pli=1

https://sustainabilitydesign.org/karlskrona-manifesto/



A dataset of national labs affiliated repositories. Good cross-validation set. https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=10564679
See dataset link in article.
